Multi-cell Coordinated Joint Sensing and Communications

This paper proposes block-level precoder (BLP) designs for a multi-input single-output (MISO) system that performs joint sensing and communication across multiple cells and users. The Cramer-Rao-Bound for estimating a target's azimuth angle is determined for coordinated beamforming (CBF) and coordinated multi-point (CoMP) scenarios while considering inter-cell communication and sensing links. The formulated optimization problems to minimize the CRB and maximize the minimum-signal-to-interference-plus-noise-ratio (SINR) are non-convex and are represented in the semidefinite relaxed (SDR) form to solve using an alternate optimization algorithm. The proposed solutions show improved performance compared to the baseline scenario that neglects the signal component from neighboring cells.

==> Secondment2/simulation_AAU/service/README <==
###############
Description:

MATLAB routines to simulate and visualize various queueing systems: 
M/M/1, M/D/1, M/G/1, M/G/infinity. Requires the "toolbox" for 
generation of random numbers. It is included in the paralel directory 
"..\ranvar". The detailed documentation can be found in 

http://www.math.uu.se/research/telecom/software/

Any suggestions or comments are welcome.

###############
Installation:

After decompressing, run servpath.m in the directory "service".
Alternatively, you may add to your startup.m:
  addpath('path_to_stsim\service', ...
          'path_to_stsim\ranvar')


###############
Version: 2.1
Last revision: 17-Dec-05

Added simstmginfty.m to simulate a stationary M/G/infinity queue, 
modified simmginfty.m.

###############
Authors: 
  Ingemar Kaj <ikaj@math.uu.se>
  Raimundas Gaigalas <jaunas@math.uu.se>

